SP2Bench: A SPARQL Performance Benchmark

Recently, the SPARQL query language for RDF has reached the W3C recommendation status. In response to this emerging standard, the database community is currently exploring efficient storage techniques for RDF data and evaluation strategies for SPARQL queries. A meaningful analysis and comparison of these approaches necessitates a comprehensive and universal benchmark platform. To this end, we have developed SP^2Bench, a publicly available, language-specific SPARQL performance benchmark. SP^2Bench is settled in the DBLP scenario and comprises both a data generator for creating arbitrarily large DBLP-like documents and a set of carefully designed benchmark queries. The generated documents mirror key characteristics and social-world distributions encountered in the original DBLP data set, while the queries implement meaningful requests on top of this data, covering a variety of SPARQL operator constellations and RDF access patterns. As a proof of concept, we apply SP^2Bench to existing engines and discuss their strengths and weaknesses that follow immediately from the benchmark results.

==> figure_documentclasses.tex <==
\begin{figure*}[t]
\hspace{-1cm}
\mbox{
\subfigure[Conferences and Journals]{\includegraphics[scale=0.5]{figures/document_classes/out/venues_per_year_plot}}
\hspace{-0.4cm}
\subfigure[Inproceedings and Articles]{\includegraphics[scale=0.5]{figures/document_classes/out/inproc-art_per_year_plot}}
\hspace{-0.4cm}
\subfigure[Other document classes]{\includegraphics[scale=0.5]{figures/document_classes/out/book-phd-masters-www-incoll_per_year_plot}}
}
\vspace{-0.65cm}
\caption{Number of document class instances starting From 1960 and approximations}
\label{fig:documentclasses}
\vspace{-0.22cm}
\end{figure*}


==> figure_inmemory.tex <==
\begin{figure*}[t]
\mbox{
\hspace{-1.7cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/inmemory/q5a}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/inmemory/q5b}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/inmemory/q6}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/inmemory/q7}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/inmemory/q12a}}}
}
\vspace{-0.4cm}
\caption{Results for in-memory engines on S1=10k, S2=50k, S3=250k, S4=1M, S5=5M, and S6=25M triples}
\label{fig:inmemory}
\vspace{-0.2cm}
\end{figure*}


==> figure_keycharacteristics.tex <==
\begin{figure*}[t]
\hspace{-0.8cm}
\mbox{
\subfigure[Characteristics of authors]{\includegraphics[scale=0.5]{figures/key_characteristics/out/author_characteristics_plot}}
\hspace{-0.4cm}
\subfigure[Distribution of publications]{\includegraphics[scale=0.5]{figures/key_characteristics/out/author_distribution_plot}}
\hspace{-0.4cm}
\subfigure[Number of incoming citations]{\includegraphics[scale=0.5]{figures/key_characteristics/out/incoming_citations_plot}}
}
\vspace{-0.6cm}
\caption{Different key characteristics found in the DBLP database}
\label{fig:miscplots}
\vspace{-0.1cm}
\end{figure*}



==> figure_native.tex <==
\begin{figure*}[t]
\mbox{
\hspace{-1.7cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/native/load}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/native/q2}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/native/q3a}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/native/q3c}}}
\hspace{-1.98cm}
\subfigure{\rotatebox{270}{\includegraphics[scale=0.22]{figures/experiments/native/q10}}}
}
\vspace{-0.4cm}
\caption{Results for physical-backend engines on S1=10k, S2=50k, S3=250k, S4=1M, S5=5M, and S6=25M triples}
\label{fig:native}
\vspace{-0.2cm}
\end{figure*}


==> figure_repeatedattributes.tex <==
\begin{figure*}[t]
\hspace{-1cm}
\mbox{
\subfigure[Distribution of citations]{
\includegraphics[scale=0.55]{figures/probability_distribution/out/distribution_cite_plot}
}
\hspace{-1.2cm}
\subfigure[Distribution of editors]{
\includegraphics[scale=0.55]{figures/probability_distribution/out/distribution_editor_plot}
}
\hspace{-1.1cm}
\subfigure[Distribution of authors]{
\includegraphics[scale=0.55]{figures/probability_distribution/out/distribution_author_plot}
}
}
\vspace{-0.6cm}
\caption{Probability distribution for repeated attribute occurrences and approximations}
\vspace{-0.2cm}
\label{fig:repeatedattributes}
\end{figure*}


==> query_discussion.tex <==
\begin{figure*}
\begin{boxedminipage}{17.7cm}
{\small

\noindent
{\bf Q1.} {\it Return the year of publication of ``Journal 1 (1940)''.}\\[-0.20cm]
\line(1,0){498}\\
\noindent
This simple query returns exactly one result (for arbitrarily large documents).
Native engines might use index lookups in order to answer this query in (almost)
constant time, i.e.~they should be independent from document size.
%\line(1,0){220}

\medskip

\noindent
{\bf Q2.} {\it Extract all inproceedings with properties
{\tt dc:creator}, {\tt bench:booktitle}, {\tt dc:title},
{\tt swrc:pages}, {\tt dcterms:partOf}, {\tt rdfs:seeAlso},
{\tt foaf:homepage}, {\tt dcterms:issued}, and optionally
{\tt bench:abstract}, including these properties.}\\[-0.20cm]
\line(1,0){498}\\
\noindent
This query implements a bushy graph pattern. It contains a single,
simple \textsc{Optional} expression, and accesses large strings
(i.e.~the abstracts). Result size grows with document size,
and a final result ordering is necessary due to operator \textsc{Order By}.
Both native and in-memory engines might reach evaluation times that are 
almost linear to the size of the document.

\medskip

\noindent
{\bf Q3abc.} {\it Select all articles with property 
(a)~{\tt swrc:pages}, (b) {\tt swrc:month}, or (c) {\tt swrc:isbn}.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
This query tests \textsc{Filter} expressions with varying
selectivity. According to Table~\ref{tbl:attributes}, the \textsc{Filter}
expression in $Q3a$ is not very selective (i.e.~selects about $92.61\%$ of
all articles). Data access through a secondary index on predicate
{\tt swrc:pages} is probably not very efficient, but might be favorable for $Q3b$,
which selects only $0.65\%$ of all articles. The filter condition in
$Q3c$ is never satisfied, since no articles have {\tt swrc:isbn} predicates.
Statistics might be used to answer $Q3c$ in constant time.

\medskip

\noindent
{\bf Q4.} {\it Select all distinct pairs of article author names for
authors that have published in the same journal.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
This query contains a long graph chain, i.e.~variables $\textit{?name1}$
and $\textit{?name2}$ are linked through their authors, the articles that
these authors published, and the common journal of both articles. The result
is very large, basically quadratic in number and size of journals. Instead of
computing the result of the outer pattern block and applying the
\textsc{Filter} afterwards, engines might factor in the \textsc{Filter}
expression in the computation of the outer block, e.g.~by exploiting indices
on the author names. Note that the \textsc{Distinct} modifier further complicates
the query.

\medskip

\noindent
{\bf Q5ab.} {\it Return the names of all persons that occur as author
of at least one inproceeding and at least one article.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
Queries $Q5a$ and $Q5b$ test different variants of joins.
$Q5a$ implements an implicit join on author names, encoded in the \textsc{Filter}
condition. In contrast, $Q5b$ explicitly joins the authors through the shared
variable $\textit{name}$. Although $Q5a$ and $Q5b$ are not equivalent in general,
they compute the same result in our scenario, due to the one-to-one mapping between
authors and their names (i.e.~author names consitute ``primary keys'').
In~\cite{lms2008}, semantic optimization on top of primary and foreign keys for
RDF has been proposed. This approach might detect the equivalence of both queries
in this scenario and select the more efficient variant.

\medskip

\noindent
{\bf Q6.} {\it Return, for each year, the set of all publications written by
authors that have not published in years before.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
$Q6$ implements closed world negation (CWN), which is expressed
through a combination of operators \textsc{Optional}, \textsc{Filter},
and \textsc{bound}. The idea of the construction is that the block outside
the \textsc{Optional} expression computes all publications, while the inner
block constitues earlier publications from authors that appear outside.
The outer \textsc{Filter} expression then retains all publications for
which $\textit{?author2}$ has not been bound, i.e.~exactly the publications
of those authors that have not published in earlier years. 

\medskip

\noindent
{\bf Q7.} {\it Return the titles of all papers that have been cited at 
least once, but not by any paper that has not been cited itself.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
This query tests double negation, which requires nested CWN.
Recalling that the citation system of DBLP is rather incomplete
(cf.~Section\ref{subsec:citations}), we expect a small number of results.
However, the query is very challenging due to the double negation.
Engines might reuse graph pattern results, for instance, the pattern 
``\verb!?class<i> rdf:type foaf:Document. ?doc<i> rdf:type ?class<i>.!''
occurs three times, for empty $i$, $i:=3$, and $i:=4$. In addition,
scenario-specific optimization might be developed.

\medskip

\noindent
{\bf Q8.} {\it Compute authors that have published directly with
``Paul Erd\"os'' or with an author that has published
with ``Paul Erd\"os''.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
Here, the evaluation of the second \textsc{Union} part is basically
``contained'' in the evaluation of the first part. Hence, techniques like
graph pattern (or subexpression) reusing might apply. Another very promising
optimization approach is to decompose the filter expressions and push down
its components, in order to decrease the size of intermediate results.


\medskip

\noindent
{\bf Q9.} {\it Return incoming and outgoing properties of persons.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
$Q9$ has been designed to test non-standard data access
patterns. Naive implementations would compute the triple patterns
of the \textsc{Union} subexpressions separately, thus evaluate
patterns where no component is bound. Then, pattern \verb!?subject ?predicate ?person!
would select all graph triples, which is rather inefficient. Another idea
is to evaluate the first triple in each \textsc{Union}
subexpression, and then use the bindings for variable $\textit{?person}$
to evaluate the second patterns more efficiently. In this case, we observe
patterns where only the $\textit{subject}$ (resp.~the $\textit{object}$)
is bound. Also observe that this query extracts schema information. Result size is
exactly $4$ (for sufficiently large documents). Statistics about
incoming and outgoing properties of $\textit{Person}$-typed
objects in native engines might be used to answer even without data access. 

\medskip

\noindent
{\bf Q10.} {\it Return all subjects that stand in any relation
to person ``Paul Erd\"os''.} In our scenario the query can be
reformulated as {\it Return publications and venues in
which ``Paul Erd\"os'' is involved either as author or as editor.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
$Q10$ implements an object bound-only access pattern, but in contrast to
$Q9$ schema statistics are not useful, since the query also returns subjects.
Recalling that ``Paul Erd\"os'' is active only between 1940 and 1996,
so result size is fixed for sufficiently large documents. Native engines
might exploit indices and reach (almost) constant execution time for
these document sizes.

\medskip

\noindent
{\bf Q11.} {\it Return (up to) 10 electronic edition URLs starting
from the 51$^{st}$ publication, in lexicographical order.}\\[-0.20cm]
\noindent
\line(1,0){498}\\
\noindent
$Q11$ focuses on the combination of solution modifiers
\textsc{Order By}, \textsc{Limit}, and \textsc{Offset}. In-memory
engines have to read, process, and sort electronic editions
prior to processing \textsc{Limit} and \textsc{Offset}.
In contrast, native engines might exploit indices and access
only a fraction of all electronic editions. Result is limited to
$10$, so these engines might reach document-independent runtimes.

\medskip

\noindent
{\bf Q12.} {\it (a) Return {\it yes} if a person occurs as author
of at least one inproceeding and one article,
{\it no} otherwise; (b) Return {\it yes} if an author
has published directly with ``Paul Erd\"os'' or with an author
that has published with ``Paul Erd\"os'', and {\it no} otherwise.}\\[-0.2cm]
\noindent
\line(1,0){498}\\
\noindent
These queries share the properties of their
\textsc{Select} counterparts $Q5a$ and $Q8$, respectively. However,
engines should break as soon as a solution has been found. They 
might even adapt the QEP, to efficiently locate a witness. For instance,
based on execution time estimations it might be favorable to evaluate the
second part of the \textsc{Union} in $Q12b$ first.
}
\end{boxedminipage}
\caption{Description and Discussion of the Benchmark Queries and Their Characteristics.}
\label{fig:query_discussion}
\end{figure*}

